LATMiX: Learnable Affine Transformations for Microscaling Quantization of LLMs

Post-training quantization (PTQ) is a widely used approach for reducing the memory and compute costs of large language models (LLMs). Recent studies have shown that applying invertible transformations to activations can significantly improve quantization robustness by reducing activation outliers; however, existing approaches are largely restricted to rotation or Hadamard-based transformations. Moreover, most studies focused primarily on traditional quantization schemes, whereas modern hardware increasingly supports the microscaling (MX) data format. Attempts to combine both showed severe performance degradation, leading prior work to introduce assumptions on the transformations. In this work, we take a complementary perspective. First, we provide a theoretical analysis of transformations under MX quantization by deriving a bound on the quantization error. Our analysis emphasizes the importance of accounting for both the activation distribution and the underlying quantization structure. Building on this analysis, we propose LATMiX, a method that generalizes outlier reduction to learnable invertible affine transformations optimized using standard deep learning tools. Experiments show consistent improvements in average accuracy for MX low-bit quantization over strong baselines on a wide range of zero-shot benchmarks, across multiple model sizes.

==> files/tables/archive/main_results_fp16_and_bf16.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table*}[t]
% \centering
% \caption{Zero-shot recovery and average accuracy on seven commonsense
% and reading-comprehension benchmarks. All methods were evaluated under the same experimental setup. Best results are highlighted in bold, and second best in underline.}
% \label{tab:benchmarks}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{llcccccc}
% \hline
% \textbf{Format} & \textbf{Method} & \textbf{Llama3.2-1B} & \begin{tabular}[c]{@{}c@{}}\textbf{Llama3.2-3B-}\\ \textbf{Instruct}
% \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Llama3.1-8B-}\\ \textbf{Instruct}\end{tabular} & \textbf{Qwen3-1.7B} & \textbf{Qwen3-4B} & \textbf{Qwen3-8B} \\ \hline
% \multirow{8}{*}{MXFP4} & RTN & 84.69 & 93.07 & 93.77 & 84.18 & 89.82 & 92.49 \\
%  & QuaRot-RTN & 82.31 & 86.46 & 80.46 & 75.15 & 86.27 & 87.98 \\
%  & GPTQ & 87.79 & 93.33 & 95.70 & 85.77 & 92.85 & 93.29 \\
%  & QuaRot & 88.68 & 94.15 & 94.95 & 87.07 & 92.00 & 94.22 \\
%  & FlatQuant & 90.52 & 93.46 & 94.92 & 89.22 & 91.42 & 96.06 \\
%  & MR-GPTQ & 91.79 & 94.21 & \underline{96.45} & 89.16 & 92.23 & 95.68 \\
%  \cdashline{2-8}
% \addlinespace[0.3em]
%  & \textbf{\MN{}-LU (Ours)} & \underline{93.15} & \textbf{96.67} & \textbf{96.58} & \textbf{93.56} & \underline{93.25} & \textbf{96.69} \\
 
%  & \textbf{\MN{}-QR (Ours)} & \textbf{94.08} & \underline{95.81} & 96.07 & \underline{89.65} & \textbf{94.38} & \underline{96.61} \\ \hline
% \multirow{8}{*}{MXINT4} & RTN & 77.16 & 87.84 & 89.81 & 76.99 & 76.12 & 85.83 \\
%  & QuaRot-RTN & 75.45 & 81.03 & 88.11 & 72.25 & 78.47 & 84.74 \\
%  & GPTQ & 77.44 & 89.11 & 86.82 & 76.47 & 83.54 & 86.93 \\
%  & QuaRot & 88.22 & 92.57 & 94.24 & 83.91 & 88.15 & 92.65 \\
%  & FlatQuant & 88.10 & 92.47 & 92.35 & 83.95 & 90.44 & 93.83 \\
%  & MR-GPTQ & 88.53 & \underline{94.34} & \textbf{95.87} & \textbf{89.00} & \underline{91.45} & 94.50 \\
%  \cdashline{2-8}
% \addlinespace[0.3em]
%  & \textbf{\MN{}-LU (Ours)} & \textbf{90.57} & \textbf{95.88} & \underline{94.90} & \underline{88.51} & 85.58 & \textbf{95.92} \\
%  & \textbf{\MN{}-QR (Ours)} & \underline{89.46} & 93.27 & 94.47 & 87.12 & \textbf{93.31} & \underline{95.10} \\ \hline
% \end{tabular}%
% }
% \end{table*}


% \begin{table*}[t]
% \centering
% \caption{Zero-shot recovery and average accuracy on seven commonsense
% and reading-comprehension benchmarks. All methods were evaluated under the same experimental setup. Best results are highlighted in bold, and second best in underline.}
% \label{tab:benchmarks}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{cccccccc}
% \hline
% \textbf{Format} & \textbf{Method} & \textbf{Llama3.2-1B} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama3.2-3B-\\ Instruct\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama3.1-8B-\\ Instruct\end{tabular}} & \textbf{Qwen3-1.7B} & \textbf{Qwen3-4B} & \textbf{Qwen3-8B} \\ \hline
% \multirow{8}{*}{MXFP4} & RTN & 84.69 & 92.98 & 93.77 & 84.18 & 85.83 & 92.49 \\
%  & QuaRot-RTN & 82.31 & 86.46 & 80.46 & 75.15 & 84.74 & 87.98 \\
%  & GPTQ & 87.79 & 93.24 & 95.70 & 85.77 & 86.93 & 93.29 \\
%  & QuaRot & 88.68 & 94.15 & 94.95 & 87.07 & 92.65 & 94.22 \\
%  & FlatQuant & 90.52 & 92.98 & 94.92 & 89.22 & 93.83 & 96.06 \\
%  & MR-GPTQ & 91.79 & 94.12 & \underline{96.45} & \underline{89.16} & 94.50 & 95.68 \\
%    \cdashline{2-8}
% \addlinespace[0.3em]
%  & \textbf{\MN{}-LU (Ours)} & \underline{93.15} & \textbf{96.67} & \textbf{96.58} & \textbf{93.56} & \textbf{95.92} & \textbf{96.69} \\
%  & \textbf{\MN{}-QR (Ours)} & \textbf{94.08} & \underline{95.72} & 96.02 & 88.32 & \underline{95.10} & \underline{96.61} \\ \hline
% \multirow{8}{*}{MXINT4} & RTN & 84.69 & 87.84 & 89.81 & 76.99 & 76.12 & 85.83 \\
%  & QuaRot-RTN & 82.31 & 81.03 & 88.11 & 72.25 & 78.47 & 84.74 \\
%  & GPTQ & 87.79 & 89.11 & 86.82 & 76.47 & 83.54 & 86.93 \\
%  & QuaRot & 88.68 & 92.57 & 94.24 & 83.91 & 88.15 & 92.65 \\
%  & FlatQuant & 90.52 & 92.47 & 92.35 & 83.95 & 90.44 & 93.83 \\
%  & MR-GPTQ & \textbf{91.79} & \underline{94.26} & \textbf{95.87} & \textbf{89.00} & \underline{91.45} & 94.50 \\
%   \cdashline{2-8}
% \addlinespace[0.3em]
%  & \textbf{\MN{}-LU (Ours)} & \underline{90.70} & \textbf{95.88} & \underline{94.90} & \underline{88.51} & 90.81 & \textbf{95.92} \\
%  & \textbf{\MN{}-QR (Ours)} & 89.46 & 93.20 & 94.47 & 88.17 & \textbf{93.48} & \underline{95.10} \\ \hline
% \end{tabular}%
% }
% \end{table*}

% \begin{table*}[t]
% \centering
% \caption{Zero-shot average recovery accuracy on seven commonsense
% and reading-comprehension benchmarks. All methods were evaluated under the same experimental setup. QuaRot and FlatQuant are combined with GPTQ quantization scheme.
% Within each model, the best method is in \textbf{bold} and the second best is \underline{underlined}.}
% \label{tab:benchmarks}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{llcccccc}
% \toprule
% \textbf{Format} & \textbf{Method} & \textbf{Llama3.2-1B} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama3.2-3B-\\ Instruct\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Llama3.1-8B-\\ Instruct\end{tabular}} & \textbf{Qwen3-1.7B} & \textbf{Qwen3-4B} & \textbf{Qwen3-8B} \\ 
% \midrule
% \multirow{8}{*}{MXFP4} & RTN & 84.69 & 92.98 & 93.77 & 84.18 & 89.80 & 92.49 \\
%  & QuaRot-RTN & 82.31 & 86.46 & 80.46 & 75.15 & 86.30 & 87.98 \\
%  & GPTQ & 87.79 & 93.24 & 95.70 & 85.77 & 92.84 & 93.29 \\
%  & QuaRot & 88.68 & 94.15 & 94.95 & 87.07 & 92.03 & 94.22 \\
%  & FlatQuant & 90.52 & 92.98 & 94.92 & 89.22 & 91.45 & 96.06 \\
%  & MR-GPTQ & 91.79 & 94.12 & \underline{96.45} & \underline{89.16} & 92.21 & 95.68 \\
%    \cdashline{2-8}
% \addlinespace[0.3em]
%  & \textbf{\MN{}-LU (Ours)} & \underline{93.15} & \textbf{96.67} & \textbf{96.58} & \textbf{93.56} & \underline{92.75} & \textbf{96.69} \\
%  & \textbf{\MN{}-QR (Ours)} & \textbf{94.08} & \underline{95.72} & 96.02 & 89.10 & \textbf{95.89} & \underline{96.61} \\ 
%  \midrule
% \multirow{8}{*}{MXINT4} & RTN & 84.69 & 87.84 & 89.81 & 76.99 & 76.12 & 85.83 \\
%  & QuaRot-RTN & 82.31 & 81.03 & 88.11 & 72.25 & 78.47 & 84.74 \\
%  & GPTQ & 87.79 & 89.11 & 86.82 & 76.47 & 83.54 & 86.93 \\
%  & QuaRot & 88.68 & 92.57 & 94.24 & 83.91 & 88.15 & 92.65 \\
%  & FlatQuant & 90.52 & 92.47 & 92.35 & 83.95 & 90.44 & 93.83 \\
%  & MR-GPTQ & \textbf{91.79} & \underline{94.26} & \textbf{95.87} & \textbf{89.00} & \underline{91.45} & 94.50 \\
%   \cdashline{2-8}
% \addlinespace[0.3em]
%  & \textbf{\MN{}-LU (Ours)} & \underline{90.70} & \textbf{95.88} & \underline{94.90} & \underline{88.51} & 90.81 & \textbf{95.92} \\
%  & \textbf{\MN{}-QR (Ours)} & 89.46 & 93.20 & 94.47 & 88.40 & \textbf{93.48} & \underline{95.10} \\ 
%  \bottomrule
% \end{tabular}%
% }
% \end{table*}


%%%%%%%%%%%%%%%%%%%%%%
% Float16 full table
%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
\caption{[FLOAT16]Zero-shot average accuracy and average recovery (in percentage) on seven commonsense
and reading-comprehension benchmarks. All methods were evaluated under the same experimental setup. QuaRot and FlatQuant are combined with GPTQ quantization scheme.
Within each model, the best method is in \textbf{bold} and the second best is \underline{underlined}.}
\label{tab:benchmarks}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{llcccccccccccc}
\toprule
\textbf{Format} & \textbf{Method}
& \multicolumn{2}{c}{\textbf{Llama3.2-1B}}
& \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama3.2-3B-\\ Instruct\end{tabular}}}
& \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama3.1-8B-\\ Instruct\end{tabular}}}
& \multicolumn{2}{c}{\textbf{Qwen3-1.7B}}
& \multicolumn{2}{c}{\textbf{Qwen3-4B}}
& \multicolumn{2}{c}{\textbf{Qwen3-8B}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}
& & Accuracy & Recovery & Accuracy & Recovery & Accuracy & Recovery
& Accuracy & Recovery & Accuracy & Recovery & Accuracy & Recovery \\
\midrule
\multirow{8}{*}{MXFP4}
& RTN &  48.75 & 84.69 &  59.54 & 92.98 & 66.84 & 93.77 &  & 84.18 & 60.19 & 89.80 &  64.83 & 92.49 \\
& QuaRot-RTN & 47.65 & 82.31 & 55.69 & 86.46 &  57.52 & 80.46 &  & 75.15 &  58.34 & 86.30 & 61.97 & 87.98 \\
& GPTQ & 50.66 & 87.79 & 59.72 & 93.24 & 68.11 & 95.70 &  & 85.77 & 62.23 & 92.84 & 65.21 & 93.29 \\
& QuaRot & 51.27 & 88.68 &  60.11 & 94.15 & 67.64 & 94.95 &  & 87.07 & 61.92 & 92.03 & 66.01 & 94.22 \\
& FlatQuant & 52.39 & 90.52 & 59.90 & 92.98 & 67.80 & 94.92 &  & 89.22 & 61.44 & 91.45 & 67.04 & 96.06 \\
& MR-GPTQ & 52.93 & 91.79 & 60.11 & 94.12 & \underline{68.59} & \underline{96.45} &  & \underline{89.16} & 61.97 & 92.21 & 67.23 & 95.68 \\
\cdashline{2-14}
\addlinespace[0.3em]
& \textbf{\MN{}-LU (Ours)} & \underline{53.79} & \underline{93.15} & \textbf{61.79} & \textbf{96.67} & \textbf{68.77} & \textbf{96.58} &  & \textbf{93.56} & \underline{62.21} & \underline{92.75} & \textbf{67.64} & \textbf{96.69} \\
& \textbf{\MN{}-QR (Ours)} & \textbf{54.08} & \textbf{94.08} & \underline{61.16} & \underline{95.72} &  68.37 & 96.02 &  & 89.10 & \textbf{64.26} & \textbf{95.89} & \underline{67.72} & \underline{96.61} \\
\midrule
\multirow{8}{*}{MXINT4}
& RTN & 44.61 & 77.16 & 55.81 & 87.84 & 64.25 & 89.81 &  & 76.99 & 50.57 & 76.12 & 60.29 & 85.83 \\
& QuaRot-RTN &  44.05 & 75.45 & 52.23 & 81.03 & 62.94 & 88.11 &  & 72.25 & 52.68 & 78.47 & 59.69 & 84.74 \\
& GPTQ & 44.51 & 77.44 & 56.88 & 89.11 & 62.08 & 86.82 &  & 76.47 & 55.95 & 83.54 & 60.99 & 86.93 \\
& QuaRot & 50.75 & 88.22 & 59.12 & 92.57 &  67.12 & 94.24 &  & 83.91 & 58.95 & 88.15 &  65.07 & 92.65 \\
& FlatQuant & 50.30 &  87.20 & 59.37 & 92.47 & 66.04 & 92.35 &  & 83.95 & 60.96 & 90.44 & 65.68 & 93.83 \\
& MR-GPTQ & 51.13 &  88.53 & \underline{60.25} & \underline{94.26} & \textbf{68.18} & \textbf{95.87} &  & \textbf{89.00} & \underline{61.58} & \underline{91.45} & 66.27 & 94.50 \\
\cdashline{2-14}
\addlinespace[0.3em]
& \textbf{\MN{}-LU (Ours)} & \textbf{52.35} & \textbf{90.70} & \textbf{61.20} & \textbf{95.88} &  \underline{67.75} & \underline{94.90} &  & \underline{88.51} & 61.04 & 90.81 & \textbf{67.18} & \textbf{95.92} \\
& \textbf{\MN{}-QR (Ours)} &  \underline{51.71} & \underline{89.46} &  59.80 & 93.20 & 67.52 & 94.47 &  & 88.40 & \textbf{62.66}  & \textbf{93.48} &  \underline{66.71} & \underline{95.10} \\
\bottomrule
\end{tabular}%
}
\end{table*}


%%%%%%%%%%%%%%%%%%%%%%
% Bfloat16 full table
%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
\centering
\caption{[BFLOAT16!!] Zero-shot average accuracy and average recovery (in percentage) on seven commonsense
and reading-comprehension benchmarks. All methods were evaluated under the same experimental setup. QuaRot and FlatQuant are combined with GPTQ quantization scheme.
Within each model, the best method is in \textbf{bold} and the second best is \underline{underlined}.}
\label{tab:benchmarks}
\resizebox{1.0\textwidth}{!}{%
\begin{tabular}{llcccccccccccc}
\toprule
\textbf{Format} & \textbf{Method}
& \multicolumn{2}{c}{\textbf{Llama3.2-1B}}
& \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama3.2-3B-\\ Instruct\end{tabular}}}
& \multicolumn{2}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Llama3.1-8B-\\ Instruct\end{tabular}}}
& \multicolumn{2}{c}{\textbf{Qwen3-1.7B}}
& \multicolumn{2}{c}{\textbf{Qwen3-4B}}
& \multicolumn{2}{c}{\textbf{Qwen3-8B}} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
\cmidrule(lr){9-10}\cmidrule(lr){11-12}\cmidrule(lr){13-14}
& & Accuracy & Recovery & Accuracy & Recovery & Accuracy & Recovery
& Accuracy & Recovery & Accuracy & Recovery & Accuracy & Recovery \\
\midrule
\multirow{8}{*}{MXFP4}
& RTN &  47.89 & 83.09 &  58.85 & 91.76 & - & - & 48.22 & 79.56 & 61.60 & 91.84 & - & - \\
& QuaRot-RTN &  48.24 & 83.38 &  55.15 & 86.00 & 58.78 & 82.35 & 45.70 & 75.47 & 59.74  & 88.66 &  61.91 & 87.86 \\
& GPTQ &  51.42 & 89.03 &  59.54 & 92.97 & - & - & 52.68 & 87.56 & 62.61  & 93.13 &  - & - \\
& QuaRot &  52.47 & 91.09 &  59.90 & 93.98 & 67.66 & 94.86 & 52.71 & 88.11 & 61.31  & 91.00 &  66.47 & 94.91 \\
& FlatQuant &  52.45 & 90.54 &  60.55 & 94.73 & 67.81 & 95.40 &54.85& 90.98 & 62.46  & 92.96 &  66.89 & 95.34 \\
& MR-GPTQ &  - & - &  60.89 & 95.37 & - & - & 52.59 & 87.34 & 62.05  & 92.02 &  - & - \\
\cdashline{2-14}
\addlinespace[0.3em]
& \textbf{\MN{}-LU (Ours)} &  \textbf{54.18} & \textbf{94.05} &  \textbf{62.25} & \textbf{97.75} & - & - & \textbf{56.91} & \textbf{94.67} & \underline{63.74}  & \underline{95.03} &  68.66 & 98.24 \\
& \textbf{\MN{}-QR (Ours)} &  \underline{52.99} & \underline{92.17} &  \underline{61.54} & \underline{96.30} & - & - & \underline{56.31} & \underline{93.56} & \textbf{64.03}  & \textbf{95.33} &  67.61 & 96.27 \\
\midrule
\multirow{8}{*}{MXINT4}
& RTN &  45.14 & 78.14 &  54.58 & 85.45 & 65.68 & 92.04 & 44.11 & 72.98 & 51.06  & 76.47 &  - & - \\
& QuaRot-RTN &  44.55 & 77.46 &  51.40 & 79.71 & 61.08 & 85.51 & 42.79 & 70.70 & 52.64  & 78.21 &  59.24 & 84.01 \\
& GPTQ &  49.06 & 85.00 &  59.25 & 92.72 & - & - & 48.47 & 80.42 & 57.00  & 85.78 &  - & - \\
& QuaRot &  49.90 & 86.30 &  58.63 & 91.76 & 66.02 & 92.54 & 49.38 & 81.98 & 59.60  & 88.42 &  65.60 & 93.42 \\
& FlatQuant &  50.34 & 87.25 &  58.31 & 90.77 & 65.81 & 91.84 & 53.12 & 88.56 & 61.50  & 91.50 &  65.80 & 93.76 \\
& MR-GPTQ &  51.37 & 89.08 &  \underline{60.82} & \underline{95.34} & 67.77 & 95.22 & 52.79 & 87.98 & 61.65  & 91.64 &  66.24 & 94.51 \\
\cdashline{2-14}
\addlinespace[0.3em]
& \textbf{\MN{}-LU (Ours)} &  \textbf{53.16} & \textbf{92.40} &  \textbf{61.10} & \textbf{95.46} & - & - & \underline{54.86} & \underline{90.77} & \underline{62.54}  & \underline{93.35} &  67.04 & 95.77 \\
& \textbf{\MN{}-QR (Ours)} &  \underline{51.84} & \underline{90.38} &  59.77 & 93.21 & - & - & \textbf{54.84} & \textbf{91.13} & \textbf{62.74}  & \textbf{93.49} &  - & - \\
\bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/eval_task_results/bfloat16_with_nvfp/llama3.1-8B-instruct.tex <==
\begin{table*}[ht]
\label{tab:llama-8b-instruct-bf16}
\caption{Performance of Llama-3.1-8B-Instruct across weight and activation quantization configurations.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Format & Method & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%)\end{tabular} \\ 
\midrule
 & FP16 &  53.58 & 75.76 & 78.51 & 76.09 & 79.49 & 83.88 & 49.00 & 70.90 & 100 \\
   \cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 50.09 & 71.68 & 74.07 & 69.14 & 78.89 & 82.26 & 43.80 & 67.13 & 94.29\\
 & QuaRot-RTN & 41.64 & 61.11 & 67.49 & 60.77 & 74.10 & 68.32 & 38.00 & 58.78 & 82.35\\
 & GPTQ & 50.60 & 73.91 & 76.90 & 72.77 & 79.27 & 80.83 & 45.20 & 68.50 & 96.27 \\
 & QuaRot & 52.05 & 74.33 & 75.91 & 70.24 & 77.58 & 82.29 & 41.20 & 67.66 & 94.86 \\
 & FlatQuant & 50.09 & 72.73 & 75.22 & 71.03 & 77.75 & 82.08 & 45.80 & 67.81 & 95.40 \\
& SpinQuant & 51.02 & 72.43 & 76.01 & 71.27 & 77.37 & 83.43 & 45.00 & 68.08 & 95.71 \\
 & MR-GPTQ & 53.67 & 76.68 & 77.08 & 72.69 & 78.35 & 82.05 & 45.60 & 69.45 & \textbf{97.79} \\
 \cdashline{2-11}
\addlinespace[0.3em]
& \textbf{\MN{}-LU (Ours) - NEW*} & 49.82 & 73.02 & 76.53 & 72.53 & 78.40 & 83.82 & 44.80 & 68.42 & 96.02 \\ 
& \textbf{\MN{}-QR (Ours) - NEW*} & 49.23 & 76.13 & 76.74 & 74.11 & 77.96 & 82.26 & 45.20 & 68.80 & 96.56  \\
\midrule
\multirow{8}{*}{MXINT4} 
& RTN & 46.25 & 71.97 & 73.35 & 67.88 & 76.39 & 80.95 & 43.00 & 65.68 & 92.04 \\
 & QuaRot-RTN & 41.98 & 64.27 & 68.88 & 62.90 & 74.43 & 74.89 & 40.20 & 61.08 & 85.51 \\
 & GPTQ & 49.15 & 72.56 & 75.79 & 70.56 & 76.93 & 79.42 & 42.40 & 66.69 & 93.54 \\
 & QuaRot & 46.25 & 69.15 & 75.99 & 67.80 & 77.86 & 81.31 & 43.80 & 66.02 & 92.54 \\
 & FlatQuant & 47.61 & 69.15 & 75.02 & 68.67 & 78.02 & 83.18 & 39.00 & 65.81 & 91.84 \\
 & SpinQuant & 49.23 & 73.61 & 76.84 & 71.43 & 78.45 & 82.11 & 44.20 & 67.98 & 95.37 \\
& MR-GPTQ & 50.26 & 73.99 & 76.65 & 70.40 & 77.80 & 80.92 & 44.40 & 67.77 & 95.22 \\
   \cdashline{2-11}
\addlinespace[0.3em]
& \textbf{\MN{}-LU (Ours) - NEW*} & 49.23 & 73.06 & 76.63 & 72.92 & 78.18 & 82.69 & 46.40 & 68.44 & \textbf{96.20} \\
& \textbf{\MN{}-QR (Ours) - NEW*} & 49.14 & 75.21 & 75.80 & 71.03 & 78.29 & 83.57 & 44.00 & 68.15 & 95.54  \\ 
  


  \midrule
\multirow{8}{*}{NVFP4} & RTN & 51.37 & 74.37 & 77.72 & 72.93 & 78.45 & 81.68 & 47.80 & 69.19 & 97.50 \\
 & QuaRot-RTN & 50.09 & 70.88 & 76.71 & 71.59 & 77.58 & 81.07 & 43.20 & 67.30 & 94.46 \\
 & GPTQ & 51.88 & 74.66 & 78.50 & 71.74 & 78.78 & 83.15 & 47.80 & \textbf{69.50} & \textbf{97.92 }\\
 & QuaRot & 51.45 & 74.66 & 77.29 & 72.61 & 79.98 & 82.66 & 45.40 & 69.15 & 97.18 \\
  & SpinQuant & 51.62 & 73.32 & 77.54 & 71.51 & 78.56 & 82.23 & 46.20 & 68.71 & 96.72 \\
 & FlatQuant & 51.96 & 74.79 & 77.48 & 72.22 & 78.56 & 81.44 & 45.40 & 68.84 & 96.84 \\
 & MR-GPTQ & 51.11 & 75.04 & 77.69 & 75.06 & 79.87 & 81.62 & 46.40 & 69.54 & 97.79 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} 
 & \textbf{\MN{}-QR (Ours)}
 \bottomrule
\end{tabular}%
}
\end{table*}




==> files/tables/eval_task_results/bfloat16_with_nvfp/llama3.2-1B.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[ht]
\label{tab:llama-1b-bf16}
\caption{Performance of Llama-3.2-1B across weight and activation quantization configurations.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Format & Method & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%)\end{tabular} \\ 
\midrule
 & FP16 & 36.86 & 61.70 & 65.79 & 62.75 & 74.81 & 63.82 & 37.00 & 57.53 & 100 \\
   \cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 29.78 & 49.37 & 52.00 & 55.88 & 66.65 & 49.94 & 31.60 & 47.89 & 83.09 \\
 & QuaRot-RTN & 28.24 & 48.40 & 47.84 & 55.72 & 66.54 & 59.54 & 31.40 & 48.24 & 83.38 \\
 & GPTQ & 31.48 & 52.61 & 57.82 & 55.88 & 69.15 & 59.97 & 33.00 & 51.42 & 89.03 \\
 & QuaRot & 33.36 & 54.76 & 56.92 & 59.12 & 69.91 & 59.60 & 33.60 & 52.47 & 91.09 \\
  & SpinQuant & 31.83 & 54.08 & 55.87 & 55.33 & 68.50 & 61.96 & 32.80 & 51.48 & 89.20 \\
 & FlatQuant & 30.89 & 55.56 & 58.57 & 57.93 & 69.26 & 62.14 & 32.80 & 52.45 & 90.54 \\
 & MR-GPTQ & 30.97 & 55.13 & 58.33 & 56.12 & 70.62 & 62.17 & 34.40 & 52.53 & 90.89 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 34.22 & 57.95 & 58.66 & 57.46 & 71.87 & 64.28 & 34.80 & \textbf{54.18} & \textbf{94.05} \\
 & \textbf{\MN{}-QR (Ours)} & 31.48 & 55.35 & 58.26 & 58.64 & 69.42 & 60.80 & 37.00 & 52.99 & 92.17\\ \midrule
\multirow{8}{*}{MXINT4} & RTN & 26.54 & 42.05 & 44.29 & 53.12 & 62.84 & 56.97 & 30.20 & 45.14 & 78.14 \\
 & QuaRot-RTN & 26.19 & 42.30 & 41.92 & 53.43 & 60.17 & 56.42 & 31.40 & 44.55 & 77.46 \\
 & GPTQ & 31.31 & 50.80 & 53.37 & 56.75 & 66.16 & 54.62 & 30.40 & 49.06 & 85.00 \\
 & QuaRot & 28.75 & 51.56 & 56.69 & 53.91 & 67.95 & 57.03 & 33.40 & 49.90 & 86.30 \\
   & SpinQuant & 30.03 & 48.57 & 54.42 & 55.88 & 65.34 & 52.51 & 31.20 & 48.28 & 83.70 \\
 & FlatQuant & 31.14 & 54.12 & 56.04 & 57.46 & 67.41 & 54.01 & 32.20 & 50.34 & 87.25 \\
 & MR-GPTQ & 32.25 & 53.62 & 56.88 & 55.09 & 69.70 & 59.08 & 33.00 & 51.37 & 89.08 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 32.94 & 58.04 & 58.27 & 56.59 & 69.31 & 61.80 & 35.20 & \textbf{53.16} & \textbf{92.40} \\
 & \textbf{\MN{}-QR (Ours)} & 33.19 & 54.63 & 57.46 & 55.41 & 68.28 & 58.72 & 35.20 & 51.84 & 90.38 \\ 

  \midrule
\multirow{8}{*}{NVFP4} & RTN &31.91 & 57.53 & 60.92 & 58.72 & 70.78 & 62.23 & 34.00 & 53.73 & 92.86 \\
 & QuaRot-RTN & 29.95 & 53.54 & 54.43 & 57.70 & 66.70 & 57.92 & 30.40 & 50.09 & 86.40 \\
 & GPTQ & 33.62 & 57.24 & 61.62 & 59.67 & 70.13 & 59.60 & 33.80 & 53.67 & 93.03 \\
 & QuaRot & 31.74 & 56.14 & 59.70 & 58.88 & 70.84 & 57.71 & 33.40 & 52.63 & 91.01 \\
  & SpinQuant & 34.64 & 57.45 & 60.52 & 59.35 & 71.49 & 61.62 & 35.40 & 54.35 & 94.49 \\
 & FlatQuant & 33.96 & 55.85 & 59.85 & 58.72 & 70.18 & 61.93 & 34.20 & 53.53 & 92.93 \\
 & MR-GPTQ& 32.85 & 58.04 & 60.06 & 55.96 & 71.55 & 59.51 & 35.20 & 53.31 & 92.52 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} 
 & \textbf{\MN{}-QR (Ours)} 
 \bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/eval_task_results/bfloat16_with_nvfp/llama3.2-3B-instruct.tex <==
\begin{table*}[ht]
\label{tab:llama-3b-instruct-bf16}
\caption{Performance of Llama3.2-3B-Instruct across weight and activation quantization configurations.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Format & Method & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%)\end{tabular} \\ 
\midrule
 & FP16 & 45.56 & 67.42 & 71.72 & 67.32 & 75.41 & 75.35 & 42.00 & 63.54 & 100 \\
   \cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 38.05 & 59.97 & 66.87 & 62.98 & 72.25 & 75.05 & 36.80 & 58.85 & 91.76
 \\
 & QuaRot-RTN & 35.67 & 53.87 & 62.30 & 61.88 & 70.67 & 67.03 & 34.60 & 55.15 & 86.00
 \\
 & GPTQ & 39.93 & 61.32 & 69.15 & 63.93 & 72.85 & 72.78 & 36.80 & 59.54 & 92.97
 \\
 & QuaRot & 41.13 & 61.45 & 68.09 & 65.35 & 73.50 & 70.58 & 39.20 & 59.90 & 93.98
 \\
& SpinQuant & 40.78 & 67.59 & 65.80 & 64.17 & 73.50 & 72.91 & 36.20 & 60.14 & 93.89
 \\
 & FlatQuant & 40.44 & 63.09 & 68.45 & 64.48 & 74.32 & 74.28 & 38.80 & 60.55 & 94.73
 \\
 & MR-GPTQ & 42.83 & 63.80 & 69.94 & 63.61 & 73.88 & 74.19 & 38.00 & 60.89 & 95.37
 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 43.09 & 65.07 & 68.87 & 64.40 & 74.65 & 78.29 & 41.40 & \textbf{62.25} & \textbf{97.75} \\
 & \textbf{\MN{}-QR (Ours)} & 43.00 & 65.53 & 69.09 & 64.88 & 75.08 & 75.20 & 38.00 & 61.54 & 96.30 \\ \midrule
\multirow{8}{*}{MXINT4} & RTN & 36.18 & 56.23 & 62.43 & 57.70 & 70.13 & 63.58 & 35.80 & 54.58 & 85.45
\\
 & QuaRot-RTN & 31.57 & 50.76 & 56.66 & 56.43 & 68.44 & 65.14 & 30.80 & 51.40 & 79.71
 \\
 & GPTQ & 40.36 & 62.67 & 67.91 & 61.09 & 71.33 & 73.82 & 37.60 & 59.25 & 92.72
 \\
 & QuaRot & 41.21 & 61.15 & 68.05 & 60.22 & 73.01 & 70.34 & 36.40 & 58.63 & 91.76
 \\
   & SpinQuant & 38.74 & 52.90 & 63.89 & 62.12 & 70.18 & 70.43 & 33.80 & 56.01 & 87.41 \\
 & FlatQuant & 39.25 & 58.54 & 66.06 & 63.93 & 72.03 & 74.13 & 34.20 & 58.31 & 90.77
 \\

 & MR-GPTQ & 43.09 & 64.90 & 68.69 & 63.85 & 73.39 & 73.61 & 38.20 & 60.82 & 95.34
 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 40.78 & 65.99 & 69.46 & 62.43 & 75.46 & 75.14 & 38.40 & \textbf{61.10} & \textbf{95.46} \\
 & \textbf{\MN{}-QR (Ours)} & 39.93 & 64.06 & 66.03 & 65.19 & 72.91 & 74.25 & 36.00 & 59.77 & 93.21 \\ 

  \midrule
\multirow{8}{*}{NVFP4} & RTN & 42.75 & 65.87 & 69.08 & 66.14 & 74.65 & 74.86 & 41.60 & 62.13 & 97.79 \\
 & QuaRot-RTN & 26.28 & 26.52 & 25.82 & 51.46 & 52.01 & 62.17 & 34.00 & 39.75 & 63.24 \\
 & GPTQ & 42.32 & 65.66 & 69.93 & 65.59 & 74.86 & 76.12 & 40.40 & 62.12 & 97.53 \\
 & QuaRot & 26.71 & 26.77 & 25.77 & 52.17 & 52.29 & 62.17 & 33.80 & 39.95 & 63.55 \\
  & SpinQuant & 43.17 & 62.96 & 70.57 & 64.48 & 74.10 & 73.30 & 40.20 & 61.26 & 96.37 \\
 & FlatQuant & 40.96 & 60.10 & 69.80 & 66.38 & 73.34 & 74.01 & 38.20 & 60.40 & 94.62 \\
 & MR-GPTQ & 41.89 & 67.30 & 70.13 & 64.80 & 74.54 & 78.23 & 40.40 & \textbf{62.47} & \textbf{97.95} \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)}
 & \textbf{\MN{}-QR (Ours)}
 
 \bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/eval_task_results/bfloat16_with_nvfp/qwen3-1.7B.tex <==
\begin{table*}[ht]
\label{tab:qwen3-1.7b-bf16}
\caption{Performance of Qwen3-1.7B across weight and activation quantization configurations.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Format & Method & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%)\end{tabular} \\ 
\midrule
 & FP16 & 43.17 & 69.57 & 60.17 & 60.38 & 72.20 & 77.61 & 37.20 & 60.04  & 100 \\
   \cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 28.33 & 45.58 & 47.81 & 54.70 & 63.38 & 67.74 & 30.00 & 48.22 & 79.56 \\
 & QuaRot-RTN & 28.16 & 40.28 & 43.19 & 55.56 & 61.64 & 63.49 & 27.60 & 45.70 & 75.47 \\
 & GPTQ & 34.73 & 54.08 & 52.17 & 55.80 & 66.27 & 71.74 & 34.00 & 52.68 & 87.56 \\
 & QuaRot & 35.84 & 52.57 & 53.69 & 55.64 & 66.27 & 69.33 & 35.60 & 52.71 & 88.11 \\
  & SpinQuant & 33.36 & 57.70 & 55.31 & 56.12 & 66.49 & 72.54 & 33.20 & 53.53 & 88.55 \\
 & FlatQuant & 36.69 & 57.58 & 56.04 & 57.06 & 68.72 & 74.07 & 33.80 & 54.85 & 90.98 \\
 & MR-GPTQ & 33.96 & 55.60 & 52.62 & 54.85 & 66.59 & 70.52 & 34.00 & 52.59 & 87.34 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 39.68 & 61.36 & 56.31 & 60.06 & 70.35 & 75.23 & 35.40 & \textbf{56.91} & \textbf{94.67} \\
 & \textbf{\MN{}-QR (Ours)} & 37.37 & 61.70 & 55.47 & 57.46 & 68.99 & 76.79 & 36.40 & 56.31 & 93.56 \\ \midrule
\multirow{8}{*}{MXINT4} & RTN & 26.11 & 39.06 & 42.74 & 49.88 & 59.03 & 63.18 & 28.80 & 44.11 & 72.98 \\
 & QuaRot-RTN & 25.43 & 35.23 & 40.47 & 52.33 & 56.42 & 62.66 & 27.00 & 42.79 & 70.70 \\
 & GPTQ & 31.14 & 48.61 & 49.21 & 52.01 & 63.49 & 64.25 & 30.60 & 48.47 & 80.42 \\
 & QuaRot & 30.63 & 45.12 & 53.81 & 53.35 & 63.28 & 67.65 & 31.80 & 49.38 & 81.98 \\
  & SpinQuant & 37.12 & 55.26 & 55.55 & 56.12 & 68.01 & 73.12 & 33.80 & 54.14 & 89.99 \\
 & FlatQuant & 34.47 & 51.68 & 54.57 & 58.64 & 67.36 & 69.91 & 35.20 & 53.12 & 88.56 \\
 & MR-GPTQ & 33.02 & 53.45 & 54.32 & 53.35 & 67.08 & 71.47 & 36.80 & 52.79 & 87.98 \\
   \cdashline{2-11}
\addlinespace[0.3em]
& \textbf{\MN{}-LU (Ours)} & 36.01 & 60.10 & 56.32 & 56.67 & 68.17 & 73.73 & 33.00 & 54.86 & 90.77 \\
 & \textbf{\MN{}-QR (Ours)} & 37.20 & 59.34 & 54.75 & 56.91 & 69.48 & 71.77 & 34.40 & \textbf{54.84} & \textbf{91.13} \\

  \midrule
\multirow{8}{*}{NVFP4} & RTN & 37.63 & 61.20 & 58.05 & 60.54 & 70.18 & 74.71 & 34.80 & 56.73 & 94.12 \\
 & QuaRot-RTN & 26.19 & 23.82 & 26.61 & 49.25 & 52.39 & 62.17 & 27.60 & 38.29 & 63.94 \\
 & GPTQ & 37.46 & 63.17 & 56.68 & 58.56 & 69.21 & 76.94 & 33.80 & 56.55 & 93.52 \\
 & QuaRot & 26.45 & 24.33 & 26.33 & 47.28 & 51.90 & 62.17 & 29.60 & 38.29 & 64.27 \\
  & SpinQuant & 34.56 & 54.88 & 56.07 & 56.27 & 68.72 & 73.70 & 34.00 & 54.03 & 89.55 \\
 & FlatQuant & 36.35 & 56.99 & 55.62 & 57.85 & 68.06 & 73.94 & 33.00 & 54.54 & 90.37 \\
 & MR-GPTQ & 38.99 & 63.22 & 56.98 & 57.38 & 69.64 & 72.23 & 37.40 & 56.55 & 94.43 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)}
 & \textbf{\MN{}-QR (Ours)} 
 \bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/eval_task_results/bfloat16_with_nvfp/qwen3-4B.tex <==
\begin{table*}[ht]
\label{tab:qwen3-4b-bf16}
\caption{Performance of Qwen3-4B across weight and activation quantization configurations.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Format & Method & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%)\end{tabular} \\ 
\midrule
 & FP16 & 53.50 & 78.41 & 70.02 & 67.01 & 74.97 & 85.02 & 40.20 & 67.02 & 100 \\
   \cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 46.59 & 70.83 & 63.99 & 63.46 & 72.36 & 76.79 & 37.20 & 61.60 & 91.84 \\
 & QuaRot-RTN & 41.30 & 68.98 & 59.35 & 61.72 & 70.29 & 80.15 & 36.40 & 59.74 & 88.66 \\
 & GPTQ & 45.14 & 71.59 & 66.13 & 61.80 & 72.63 & 82.60 & 38.40 & 62.61 & 93.13 \\
 & QuaRot & 45.31 & 69.95 & 63.90 & 62.90 & 71.11 & 80.40 & 35.60 & 61.31 & 91.00 \\
  & SpinQuant & 43.00 & 73.32 & 63.52 & 62.27 & 70.84 & 80.98 & 39.00 & 61.85 & 92.04 \\
 & FlatQuant & 46.84 & 70.37 & 64.87 & 61.96 & 72.63 & 82.78 & 37.80 & 62.46 & 92.96 \\
 & MR-GPTQ & 45.31 & 68.73 & 64.15 & 64.25 & 72.14 & 83.76 & 36.00 & 62.05 & 92.02 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 48.29 & 73.95 & 64.84 & 63.61 & 72.74 & 83.33 & 39.40 & 63.74 & 95.03 \\
 % & \textbf{\MN{}-LU (Ours) - NEW} & 48.03 & 73.10 & 65.63 & 65.50 & 72.95 &  83.54 & 39.20 & 63.99 & 95.47 \\
 & \textbf{\MN{}-QR (Ours)} & 48.55 & 74.07 & 65.98 & 63.38 & 73.67 & 83.73 & 38.80 & \textbf{64.03} & \textbf{95.33} \\ 
 % & \textbf{\MN{}-QR (Ours) - NEW} & 46.07 & 71.50 & 64.98 & 63.61 & 74.91 & 82.56 & 38.20 & 63.12 & 94.18 \\
 % & \textbf{\MN{}-QR (Ours) - NEW [t=1]} & 46.50 & 71.80 & 65.38 & 63.93 & 72.74 & 78.86 & 38.80 & 62.57 & 93.36 \\
 \midrule
\multirow{8}{*}{MXINT4} & RTN & 33.70 & 49.33 & 54.44 & 54.22 & 67.74 & 63.58 & 34.40 & 51.06 & 76.47 \\
 & QuaRot-RTN & 34.04 & 52.69 & 54.56 & 55.64 & 65.83 & 72.51 & 33.20 & 52.64 & 78.21 \\
 & GPTQ & 40.78 & 60.23 & 61.23 & 62.27 & 70.84 & 65.08 & 38.60 & 57.00 & 85.78 \\
 & QuaRot & 44.45 & 67.63 & 62.65 & 61.56 & 68.93 & 77.98 & 34.00 & 59.60 & 88.42 \\
  & SpinQuant & 43.94 & 69.11 & 65.12 & 61.25 & 73.45 & 68.93 & 39.20 & 60.14 & 90.18 \\
 & FlatQuant & 42.32 & 71.38 & 63.76 & 61.64 & 71.22 & 81.41 & 38.80 & 61.50 & 91.50 \\
 & MR-GPTQ & 44.88 & 69.44 & 63.93 & 63.14 & 71.87 & 81.25 & 37.00 & 61.65 & 91.64 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 46.42 & 70.45 & 66.36 & 63.93 & 73.39 & 78.44 & 38.80 & 62.54 & 93.35 \\
 % & \textbf{\MN{}-LU (Ours) - NEW} & 44.53 &  &  &  &  &  &  &  &  \\
 % & \textbf{\MN{}-LU (Ours) - NEW} & 48.54 & 71.96 & 65.56 & 61.48 & 73.55 & 82.11 & 39.60 & 63.26 & 94.38 \\
 & \textbf{\MN{}-QR (Ours)} & 47.27 & 72.60 & 65.10 & 62.19 & 72.69 & 80.95 & 38.40 & \textbf{62.74} & \textbf{93.49} \\ 
  % & \textbf{\MN{}-QR (Ours) - NEW} &  & 69.78 &  & 62.74 & 73.12 & 76.20 & 39.20 &  &  \\
  % & \textbf{\MN{}-QR (Ours) - NEW} & 45.56 & 72.05 & 65.89 & 63.22 & 72.30 & 80.67 & 38.40 & 62.58 & 93.37 \\

 \midrule
\multirow{8}{*}{NVFP4} & RTN & 48.38 & 73.19 & 67.81 & 65.11 & 74.10 & 82.75 & 37.60 & 64.13 & 95.36 \\
 & QuaRot-RTN &  &  &  &  &  &  &  &  &  \\
 & GPTQ & 49.74 & 73.65 & 67.98 & 65.51 & 73.12 & 82.97 & 38.20 & 64.45 & 95.99 \\
 & QuaRot &  &  &  &  &  &  &  &  &  \\
  & SpinQuant & 44.37 & 68.90 & 64.67 & 62.75 & 71.33 & 83.24 & 36.00 & 61.61 & 91.34 \\
 & FlatQuant & 46.67 & 69.44 & 65.96 & 62.43 & 72.25 & 83.43 & 38.80 & 62.71 & 93.46 \\
 & MR-GPTQ & 47.95 & 70.66 & 65.88 & 64.09 & 71.60 & 83.03 & 37.00 & 62.89 & 93.53 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)}
 & \textbf{\MN{}-QR (Ours)} 
 
 \bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/eval_task_results/bfloat16_with_nvfp/qwen3-8B.tex <==
\begin{table*}[ht]
\label{tab:qwen3-8b-bf16}
\caption{Performance of Qwen3-8B across weight and activation quantization configurations.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Format & Method & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%)\end{tabular} \\ 
\midrule
 & FP16 & 56.74 & 80.68 & 76.53 & 70.17 & 77.69 & 86.64 & 41.60 & 70.01 & 100 \\
   \cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 45.14 & 69.32 & 69.25 & 65.59 & 73.23 & 80.00 & 38.20 & 62.96 & 89.69 \\
 & QuaRot-RTN & 46.25 & 67.76 & 67.19 & 64.64 & 72.63 & 80.12 & 34.80 & 61.91 & 87.86 \\
 & GPTQ & 49.57 & 75.00 & 70.62 & 65.59 & 74.59 & 83.76 & 40.60 & 65.68 & 93.77 \\
 & QuaRot & 50.68 & 75.55 & 72.05 & 66.14 & 74.81 & 85.05 & 41.00 & 66.47 & 94.91 \\
  & SpinQuant & 52.30 & 74.62 & 71.63 & 66.46 & 77.53 & 84.80 & 41.40 & 66.96 & 95.74 \\
 & FlatQuant & 52.13 & 76.09 & 72.55 & 68.03 & 75.41 & 84.62 & 39.40 & 66.89 & 95.34 \\
 & MR-GPTQ & 52.73 & 78.41 & 72.73 & 67.25 & 75.84 & 84.83 & 41.20 & 67.57 & 96.51 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 54.69 & 77.57 & 74.06 & 69.93 & 76.33 & 85.81 & 42.20 & \textbf{68.66} & \textbf{98.24 }\\
  % & \textbf{\MN{}-LU (Ours) - NEW} & 52.47 & 78.15 & 72.80 & 68.35 & 76.49 & 84.34 & 40.20 & 67.54 & 96.47 \\
 & \textbf{\MN{}-QR (Ours)} & 54.95 & 78.70 & 72.91 & 68.11 & 76.12 & 84.95 & 40.80 & 68.08 & 97.26 \\
 % & \textbf{\MN{}-QR (Ours) - NEW} & 53.15 & 75.21 & 72.52 & 68.19 & 75.29 & 84.03 & 40.80 & 67.03 & 95.74 \\
 % & \textbf{\MN{}-QR (Ours) - NEW [t=1]} & 51.36 & 74.53 & 71.69 & 67.87 & 75.51 & 84.15 & 40.40 & 66.50 & 94.98 \\
 \midrule
\multirow{8}{*}{MXINT4} & RTN & 42.75 & 66.25 & 64.73 & 59.19 & 71.76 & 73.88 & 35.60 & 59.17 & 84.23 \\
 & QuaRot-RTN & 40.70 & 65.45 & 65.38 & 61.88 & 72.47 & 74.62 & 34.20 & 59.24 & 84.01 \\
 & GPTQ & 43.86 & 67.63 & 67.37 & 64.96 & 72.58 & 80.40 & 37.80 & 62.08 & 88.40 \\
 & QuaRot & 50.77 & 75.13 & 71.09 & 67.48 & 75.24 & 81.50 & 38.00 & 65.60 & 93.42 \\
  & SpinQuant & 50.43 & 71.38 & 73.11 & 65.90 & 75.68 & 82.02 & 39.80 & 65.47 & 93.51 \\
 & FlatQuant & 48.55 & 74.92 & 70.98 & 67.01 & 75.57 & 83.76 & 39.80 & 65.80 & 93.76 \\
 & MR-GPTQ & 49.15 & 74.24 & 72.01 & 68.82 & 75.79 & 83.27 & 40.40 & 66.24 & 94.51 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 50.09 & 75.88 & 74.12 & 67.17 & 75.84 & 84.40 & 41.80 & \textbf{67.04} & \textbf{95.77} \\
 & \textbf{\MN{}-QR (Ours)}& 52.73 & 76.01 & 71.23 & 67.25 & 76.39 & 83.24 & 39.60 & 66.64 & 95.09 \\ 

  \midrule
\multirow{8}{*}{NVFP4} & RTN & 55.20 & 78.83 & 74.44 & 68.51 & 76.06 & 86.09 & 41.60 & \textbf{68.68} & \textbf{98.17} \\
 & QuaRot-RTN & 25.34 & 24.83 & 26.43 & 48.70 & 52.07 & 49.08 & 29.40 & 36.55 & 53.39 \\
 & GPTQ & 55.20 & 79.55 & 74.29 & 67.01 & 76.39 & 86.36 & 41.80 & 68.66 & 98.13 \\

 & QuaRot & 27.47 & 24.79 & 26.23 & 51.38 & 51.14 & 49.20 & 28.00 & 36.89 & 53.80 \\
  & SpinQuant & 53.75 & 77.40 & 73.05 & 68.03 & 75.08 & 85.75 & 39.60 & 67.52 & 96.27 \\
 & FlatQuant & 51.79 & 78.75 & 73.23 & 67.56 & 76.50 & 85.84 & 42.00 & 67.95 & 97.05 \\
 & MR-GPTQ & 55.12 & 78.91 & 74.22 & 68.59 & 76.33 & 85.41 & 41.60 & 68.60 & 98.07 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)}
 & \textbf{\MN{}-QR (Ours)}
 
 \bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/eval_task_results/float16/llama3.1-8B-instruct.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[ht]
\label{tab:llama-8b-instruct}
\caption{Performance of Llama-3.1-8B-Instruct across weight and activation quantization configurations.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Format & Method & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%)\end{tabular} \\ 
\midrule
 & FP16 & 53.92 & 75.88 & 78.44 & 75.61 & 79.54 & 83.76 & 49.20 & 70.91 & 100 \\
 \cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 48.55 & 71.17 & 74.99 & 70.48 & 77.58 & 81.10 & 44.00 & 66.84 & 93.77 \\
 & QuaRot-RTN & 39.25 & 58.75 & 66.28 & 61.09 & 73.78 & 66.12 & 37.40 & 57.52 & 80.46 \\
 & GPTQ & 49.15 & 73.99 & 76.14 & 71.59 & 78.24 & 81.44 & 46.20 & 68.11 & 95.70 \\
 & QuaRot & 50.43 & 75.25 & 75.83 & 70.01 & 75.90 & 82.29 & 43.80 & 67.64 & 94.95 \\
 & SpinQuant & 50.68 & 72.26 & 77.12 & 73.80 & 77.91 & 82.66 & 43.20 & 68.23 & 95.65 \\
 & FlatQuant & 48.12 & 73.19 & 76.71 & 70.64 & 78.02 & 84.13 & 43.80 & 67.80 & 94.92 \\
 & MR-GPTQ & 52.99 & 74.66 & 76.72 & 72.77 & 77.69 & 80.89 & 44.40 & 68.59 & 96.45 \\
 \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 50.09 & 72.85 & 76.99 & 71.98 & 78.89 & 84.37 & 46.20 & \textbf{68.77} & \textbf{96.58} \\
 & \textbf{\MN{}-QR (Ours)} & 49.23 & 73.86 & 75.84 & 72.53 & 78.07 & 82.81 & 46.20 & 68.37 & 96.02 \\ 
 \midrule
\multirow{8}{*}{MXINT4} & RTN & 45.56 & 70.03 & 72.64 & 68.35 & 74.81 & 78.35 & 40.00 & 64.25 & 89.81 \\
 & QuaRot-RTN & 44.62 & 68.64 & 70.59 & 63.14 & 74.76 & 78.01 & 40.80 & 62.94 & 88.11 \\
 & GPTQ & 41.38 & 63.76 & 67.47 & 65.90 & 76.50 & 77.95 & 41.60 & 62.08 & 86.82 \\
 & QuaRot & 49.06 & 71.25 & 76.66 & 69.85 & 77.58 & 80.83 & 44.60 & 67.12 & 94.24 \\
  & SpinQuant & 49.91 & 75.97 & 74.93 & 71.35 & 78.62 & 78.10 & 45.80 & 67.81 & 95.39 \\
 & FlatQuant & 46.33 & 71.25 & 75.03 & 70.32 & 77.42 & 80.12 & 41.80 & 66.04 & 92.35 \\
 & MR-GPTQ & 50.77 & 74.07 & 75.99 & 70.48 & 78.18 & 81.99 & 45.80 & \textbf{68.18} & \textbf{95.87} \\
 \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 48.12 & 74.58 & 76.71 & 72.45 & 78.62 & 80.18 & 43.60 & 67.75 & 94.90 \\
 & \textbf{\MN{}-QR (Ours)} & 46.93 & 73.53 & 76.67 & 71.43 & 77.64 & 82.84 & 43.60 & 67.52 & 94.47 \\ 
 \bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/eval_task_results/float16/llama3.2-1B.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[ht]
\label{tab:llama-1b}
\caption{Performance of Llama-3.2-1B across weight and activation quantization configurations.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Format & Method & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%)\end{tabular} \\ 
\midrule
 & FP16 & 36.60 & 61.83 & 65.88 & 63.30 & 74.76 & 63.76 & 37.20 & 57.62 & 100 \\
   \cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 30.03 & 50.00 & 52.05 & 54.38 & 66.59 & 54.56 & 33.60 & 48.75 & 84.69 \\
 & QuaRot-RTN & 28.58 & 47.31 & 49.05 & 54.93 & 65.83 & 57.03 & 30.80 & 47.65 & 82.31 \\
 & GPTQ & 30.46 & 52.27 & 55.32 & 54.85 & 68.28 & 59.24 & 34.20 & 50.66 & 87.79 \\
 & QuaRot & 31.48 & 54.25 & 57.68 & 56.59 & 69.70 & 56.18 & 33.00 & 51.27 & 88.68 \\
 & SpinQuant & 31.82 & 51.13 & 55.86 & 58.08 & 67.62 & -- & 32.40 & -- & -- \\
 & FlatQuant & 30.72 & 52.61 & 58.01 & 58.25 & 70.02 & 62.75 & 34.40 & 52.39 & 90.52 \\
 & MR-GPTQ & 33.45 & 55.51 & 58.36 & 59.19 & 69.42 & 60.58 & 34.00 & 52.93 & 91.79 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 32.85 & 57.70 & 59.94 & 57.54 & 70.02 & 63.67 & 34.80 & 53.79 & 93.15 \\
 & \textbf{\MN{}-QR (Ours)} & 33.96 & 58.12 & 58.75 & 58.88 & 70.35 & 61.90 & 36.60 & \textbf{54.08} & \textbf{94.08} \\ \midrule
\multirow{8}{*}{MXINT4} & RTN & 27.13 & 43.60 & 44.47 & 52.17 & 62.51 & 53.21 & 29.20 & 44.61 & 77.16 \\
 & QuaRot-RTN & 24.23 & 44.07 & 42.72 & 52.96 & 60.72 & 57.03 & 26.60 & 44.05 & 75.45 \\
 & GPTQ & 29.95 & 43.18 & 45.17 & 51.70 & 60.94 & 51.80 & 28.80 & 44.51 & 77.44 \\
 & QuaRot & 30.46 & 53.45 & 55.94 & 55.80 & 67.79 & 56.02 & 35.80 & 50.75 & 88.22 \\
 & FlatQuant & 29.35 & 50.25 & 53.87 & 57.70 & 66.70 & 59.45 & 34.80 & 50.30 & 87.20 \\
 & MR-GPTQ & 31.66 & 52.10 & 57.02 & 55.56 & 68.17 & 60.40 & 33.00 & 51.13 & 88.53 \\
   \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 30.97 & 55.22 & 58.97 & 57.22 & 69.86 & 59.39 & 34.80 & \textbf{52.35} & \textbf{90.70} \\
 & \textbf{\MN{}-QR (Ours)} & 30.80 & 54.17 & 56.13 & 56.20 & 67.74 & 63.15 & 33.80 & 51.71 & 89.46 \\ 
 \bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/eval_task_results/float16/llama3.2-3B-instruct.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[ht]
\label{tab:llama-3b-instruct}
\caption{Performance of Llama-3.2-3B-Instruct across weight and activation quantization configurations.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Format & Method & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%)\end{tabular} \\ 
\midrule
 & FP16 & 45.22 & 67.09 & 71.60 & 67.25 & 75.46 & 76.36 & 42.20 & 63.60 & 100 \\
  \cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 40.78 & 61.49 & 67.36 & 63.77 & 72.74 & 74.07 & 36.60 & 59.54 & 92.98 \\
 & QuaRot-RTN & 33.87 & 53.16 & 63.28 & 60.85 & 71.44 & 72.23 & 35.00 & 55.69 & 86.46 \\
 & GPTQ & 39.76 & 63.13 & 67.34 & 65.11 & 72.85 & 72.63 & 37.20 & 59.72 & 93.24 \\
 & QuaRot & 41.47 & 61.28 & 67.94 & 62.59 & 73.18 & 75.32 & 39.00 & 60.11 & 94.15 \\
 & FlatQuant & 40.10 & 63.17 & 68.18 & 64.72 & 73.01 & 73.27 & 36.80 & 59.90 & 92.98 \\
 & MR-GPTQ & 41.64 & 64.06 & 69.65 & 62.83 & 74.27 & 70.37 & 38.00 & 60.11 & 94.12 \\
  \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 42.06 & 64.56 & 69.02 & 66.22 & 73.72 & 77.52 & 39.40 & \textbf{61.79} & \textbf{96.67} \\
 & \textbf{\MN{}-QR (Ours)} & 42.75 & 65.95 & 67.46 & 63.93 & 74.27 & 75.60 & 38.20 & 61.16 & 95.72 \\ 
 \midrule
\multirow{8}{*}{MXINT4} & RTN & 37.12 & 55.47 & 63.89 & 58.41 & 70.95 & 65.05 & 39.80 & 55.81 & 87.84 \\
 & QuaRot-RTN & 32.42 & 51.89 & 57.09 & 55.25 & 69.21 & 67.77 & 32.00 & 52.23 & 81.03 \\
 & GPTQ & 39.68 & 54.34 & 65.22 & 60.69 & 71.44 & 70.43 & 36.40 & 56.88 & 89.11 \\
 & QuaRot & 40.70 & 63.05 & 67.64 & 62.51 & 71.93 & 70.40 & 37.60 & 59.12 & 92.57 \\
 & FlatQuant & 38.74 & 63.55 & 67.20 & 63.69 & 72.58 & 73.61 & 36.20 & 59.37 & 92.47 \\
 & MR-GPTQ & 42.41 & 63.17 & 69.12 & 64.17 & 74.21 & 71.68 & 37.00 & 60.25 & 94.26 \\
  \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 43.09 & 64.52 & 68.60 & 64.01 & 74.43 & 74.95 & 38.80 & \textbf{61.20} & \textbf{95.88} \\
 & \textbf{\MN{}-QR (Ours)} & 37.97 & 59.85 & 67.37 & 63.38 & 73.39 & 78.01 & 38.60 & 59.80 & 93.20 \\ 
 \bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/eval_task_results/float16/qwen3-1.7B.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[ht]
\label{tab:qwen-1.7b}
\caption{Performance of Qwen3-1.7B across weight and activation quantization configurations.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Format & Method & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%)\end{tabular} \\ 
\midrule
 & FP16 & 43.00 & 69.78 & 60.25 & 60.54 & 72.14 & 77.55 & 37.20 & 60.07 & 100 \\ 
 \cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 32.51 & 52.06 & 51.94 & 56.59 & 65.61 & 65.17 & 31.40 & 50.76 & 84.18 \\
 & QuaRot-RTN & 26.62 & 40.91 & 42.98 & 53.43 & 60.94 & 63.52 & 29.60 & 45.43 & 75.15 \\
 & GPTQ & 32.17 & 52.19 & 50.89 & 58.33 & 67.85 & 65.96 & 33.80 & 51.60 & 85.77 \\
 & QuaRot & 34.98 & 51.89 & 53.53 & 57.62 & 68.17 & 69.63 & 31.80 & 52.52 & 87.07 \\
 & FlatQuant & 36.77 & 54.80 & 54.82 & 55.64 & 66.92 & 73.30 & 33.60 & 53.69 & 89.22 \\
 & MR-GPTQ & 33.70 & 57.32 & 53.73 & 58.41 & 68.06 & 72.72 & 33.40 & 53.91 & 89.16 \\
 \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 40.19 & 60.14 & 54.64 & 56.35 & 69.70 & 75.69 & 36.20 & \textbf{56.13} & \textbf{93.56} \\
 & \textbf{\MN{}-QR (Ours)} & 34.90 & 57.24 & 54.01 & 57.30 & 67.52 & 71.07 & 31.80 & 53.41 & 88.32 \\ 
 \midrule
\multirow{8}{*}{MXINT4} & RTN & 28.50 & 46.25 & 46.23 & 54.62 & 62.19 & 58.81 & 28.80 & 46.48 & 76.99 \\
 & QuaRot-RTN & 24.49 & 36.91 & 41.98 & 53.75 & 58.43 & 63.79 & 27.60 & 43.85 & 72.25 \\
 & GPTQ & 29.86 & 44.70 & 47.21 & 50.91 & 62.02 & 55.54 & 30.40 & 45.81 & 76.47 \\
 & QuaRot & 30.89 & 46.72 & 53.54 & 55.25 & 65.18 & 68.07 & 33.60 & 50.46 & 83.91 \\
 & FlatQuant & 32.34 & 48.86 & 53.48 & 57.06 & 65.45 & 65.75 & 31.20 & 50.59 & 83.95 \\
 & MR-GPTQ & 34.81 & 59.18 & 54.36 & 55.49 & 67.90 & 69.66 & 34.00 & \textbf{53.63} & \textbf{89.00} \\
 \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 34.73 & 55.72 & 54.75 & 57.46 & 68.23 & 69.30 & 33.20 & 53.34 & 88.51 \\
 & \textbf{\MN{}-QR (Ours)} & 35.75 & 55.09 & 51.88 & 57.70 & 66.16 & 67.31 & 35.40 & 52.76 & 88.17 \\ 
 \bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/eval_task_results/float16/qwen3-4B.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[ht]
\label{tab:qwen-4b}
\caption{Performance of Qwen3-4B across weight and activation quantization configurations.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
Format & Method & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%)\end{tabular} \\ 
\midrule
 & FP16 & 54.10 & 78.54 & 70.08 & 66.46 & 74.97 & 85.11 & 40.00 & 67.03 & 100 \\ 
\cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 43.09 & 66.20 & 64.64 & 61.56 & 71.06 & 77.00 & 37.80 & 60.19 & 89.80 \\
 & QuaRot-RTN & 40.02 & 66.37 & 59.62 & 60.30 & 69.59 & 78.72 & 33.80 & 58.34 & 86.30 \\
 & GPTQ & 46.16 & 69.78 & 65.63 & 62.04 & 71.65 & 81.35 & 39.00 & 62.23 & 92.84 \\
 & QuaRot & 46.67 & 70.62 & 63.66 & 63.38 & 71.55 & 81.16 & 36.40 & 61.92 & 92.03 \\
 & FlatQuant & 46.08 & 67.51 & 65.74 & 63.22 & 70.95 & 79.97 & 36.60 & 61.44 & 91.45 \\
 & MR-GPTQ & 44.97 & 70.71 & 63.29 & 62.98 & 70.51 & 83.12 & 38.20 & 61.97 & 92.21 \\
\cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 46.84 & 69.36 & 64.72 & 63.61 & 71.71 & 81.22 & 38.00 & 62.21 & 92.75 \\
 & \textbf{\MN{}-QR (Ours)} & 49.32 & 75.00 & 66.28 & 62.98 & 73.56 & 82.91 & 39.80 & \textbf{64.26} & \textbf{95.89} \\ \midrule
\multirow{8}{*}{MXINT4} & RTN & 35.15 & 49.83 & 55.15 & 53.99 & 68.88 & 56.57 & 34.40 & 50.57 & 76.12 \\
 & QuaRot-RTN & 36.43 & 54.84 & 54.44 & 55.25 & 66.76 & 68.01 & 33.00 & 52.68 & 78.47 \\
 & GPTQ & 38.74 & 56.61 & 60.83 & 57.06 & 72.31 & 70.52 & 35.60 & 55.95 & 83.54 \\
 & QuaRot & 44.88 & 67.59 & 62.47 & 60.38 & 69.37 & 71.19 & 36.80 & 58.95 & 88.15 \\
 & FlatQuant & 44.37 & 70.75 & 64.16 & 61.72 & 71.65 & 78.44 & 35.60 & 60.96 & 90.44 \\
 & MR-GPTQ & 45.56 & 70.83 & 64.79 & 62.83 & 71.82 & 79.42 & 35.80 & 61.58 & 91.45 \\
 \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 44.88 & 70.16 & 63.95 & 61.40 & 71.98 & 78.29 & 36.60 & 61.04 & 90.81 \\
 & \textbf{\MN{}-QR (Ours)} & 46.42 & 71.76 & 65.05 & 64.17 & 72.36 & 80.06 & 38.80 & \textbf{62.66} & \textbf{93.48} \\ \bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/eval_task_results/float16/qwen3-8B.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% \begin{table*}[t]
% \centering
% \caption{Zero-shot accuracy for Qwen3-8B across seven commonsense and reading-comprehension benchmarks under MXFP4 and MXINT4 weight-activation quantization formats, comparing different quantization methods within each format. Within each benchmark, the best method is \textbf{bolded} and the second best is \underline{underlined}.}
% \caption{Performance of Qwen3-8B across weight and activation quantization configurations.}
% \label{tab:qwen-8b}
% \resizebox{0.9\textwidth}{!}{%
% \begin{tabular}{llccccccccc}
% \toprule
% \textbf{Format} & \textbf{Method} & \textbf{ARC-C} & \textbf{ARC-E} & \textbf{HellaSwag} & \textbf{WinoGrande} & \textbf{PIQA} & \textbf{BOOLQ} & \textbf{OBQA} & \textbf{Avg.} & \textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery \% \end{tabular}} \\ 
% \midrule
%  & FP16 & 56.40 & 80.89 & 76.46 & 70.56 & 77.80 & 86.61 & 41.40 & 70.02 & 100 \\
%  \cline{2-11}
% \addlinespace[0.3em]
% \multirow{8}{*}{MXFP4} & RTN & 49.23 & 73.57 & 70.22 & 64.56 & 73.56 & 83.24 & 39.40 & 64.83 & 92.49 \\
%  & QuaRot-RTN & 45.05 & 66.96 & 67.65 & 65.35 & 72.91 & 80.46 & 35.40 & 61.97 & 87.98 \\
%  & GPTQ & 47.70 & 73.19 & 70.21 & 64.17 & 74.32 & 84.68 & 42.20 & 65.21 & 93.29 \\
%  & QuaRot & 50.26 & 74.83 & 72.18 & 66.14 & 74.16 & 84.31 & 40.20 & 66.01 & 94.22 \\
%  & FlatQuant & 52.47 & 74.58 & 71.98 & \textbf{68.03} & \underline{76.12} & 83.91 & \textbf{42.20} & 67.04 & 96.06 \\
%  & MR-GPTQ & 52.73 & \underline{77.95} & 72.57 & \underline{67.40} & 75.79 & \textbf{85.57} & 38.60 & 67.23 & 95.68 \\
%  \cdashline{2-11}
% \addlinespace[0.3em]
%  & \textbf{\MN{}-LU (Ours)} & \textbf{55.46} & 76.77 & \underline{72.81} & 66.93 & 75.84 & \underline{85.23} & \underline{40.40} & \textbf{67.64} & \textbf{96.69} \\
%  & \textbf{\MN{}-QR (Ours)} & \underline{54.35} & \textbf{78.91} & \textbf{73.41} & 67.32 & \textbf{76.55} & 83.91 & 39.60 & \underline{67.72} & \underline{96.61} \\ 
%  \midrule
% \multirow{8}{*}{MXINT4} & RTN & 44.20 & 66.16 & 66.21 & 61.40 & 72.09 & 76.15 & 35.80 & 60.29 & 85.83 \\
%  & QuaRot-RTN & 41.81 & 65.49 & 65.98 & 61.56 & 71.71 & 76.48 & 34.80 & 59.69 & 84.74 \\
%  & GPTQ & 43.34 & 67.00 & 66.37 & 61.09 & 72.25 & 79.05 & 37.80 & 60.99 & 86.93 \\
%  & QuaRot & 47.70 & 74.41 & 70.82 & 65.35 & 75.14 & 83.09 & 39.00 & 65.07 & 92.65 \\
%  & FlatQuant & 50.17 & 72.94 & 71.71 & 65.82 & 74.54 & \textbf{84.19} & \textbf{40.40} & 65.68 & 93.83 \\
%  & MR-GPTQ & 51.79 & \textbf{76.56} & 72.28 & 65.67 & 75.19 & 83.21 & 39.20 & 66.27 & 94.50 \\
%  \cdashline{2-11}
% \addlinespace[0.3em]
%  & \textbf{\MN{}-LU (Ours)} & \underline{52.73} & 75.55 & \textbf{72.76} & \textbf{69.22} & \textbf{76.22} & \underline{83.76} & \underline{40.00} & \textbf{67.18} & \textbf{95.92} \\
%  & \textbf{\MN{}-QR (Ours)} & \textbf{53.16} & \underline{75.80} & \underline{72.45} & \underline{68.51} & \underline{75.79} & 82.91 & 38.40 & \underline{66.71} & \underline{95.10} \\ 
%  \bottomrule
% \end{tabular}%
% }
% \end{table*}

\begin{table*}[ht]
\centering
\caption{Performance of Qwen3-8B across weight and activation quantization configurations.}
\label{tab:qwen-8b}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccccc}
\toprule
\textbf{Format} & \textbf{Method} & ARC-C & ARC-E & HellaSwag & WinoGrande & PIQA & BOOLQ & OBQA & \begin{tabular}[c]{@{}c@{}}Avg.\\ Accuracy\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg.\\ Recovery (\%) \end{tabular} \\ 
\midrule
 & FP16 & 56.40 & 80.89 & 76.46 & 70.56 & 77.80 & 86.61 & 41.40 & 70.02 & 100 \\
 \cline{2-11}
\addlinespace[0.3em]
\multirow{8}{*}{MXFP4} & RTN & 49.23 & 73.57 & 70.22 & 64.56 & 73.56 & 83.24 & 39.40 & 64.83 & 92.49 \\
 & QuaRot-RTN & 45.05 & 66.96 & 67.65 & 65.35 & 72.91 & 80.46 & 35.40 & 61.97 & 87.98 \\
 & GPTQ & 47.70 & 73.19 & 70.21 & 64.17 & 74.32 & 84.68 & 42.20 & 65.21 & 93.29 \\
 & QuaRot & 50.26 & 74.83 & 72.18 & 66.14 & 74.16 & 84.31 & 40.20 & 66.01 & 94.22 \\
 & FlatQuant & 52.47 & 74.58 & 71.98 & 68.03 & 76.12 & 83.91 & 42.20 & 67.04 & 96.06 \\
& SpinQuant & 50.51 & 73.48 & 72.27 & 66.85 & 76.33 & 84.22 & 40.80 & 66.35 & 94.80 \\
 & MR-GPTQ & 52.73 & 77.95 & 72.57 & 67.40 & 75.79 & 85.57 & 38.60 & 67.23 & 95.68 \\
 \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 55.46 & 76.77 & 72.81 & 66.93 & 75.84 & 85.23 & 40.40 & \textbf{67.64} & \textbf{96.69} \\
 & \textbf{\MN{}-QR (Ours)} & 54.35 & 78.91 & 73.41 & 67.32 & 76.55 & 83.91 & 39.60 & 67.72 & 96.61 \\ 
 \midrule
\multirow{8}{*}{MXINT4} & RTN & 44.20 & 66.16 & 66.21 & 61.40 & 72.09 & 76.15 & 35.80 & 60.29 & 85.83 \\
 & QuaRot-RTN & 41.81 & 65.49 & 65.98 & 61.56 & 71.71 & 76.48 & 34.80 & 60.29 & 85.83 \\
 & GPTQ & 43.34 & 67.00 & 66.37 & 61.09 & 72.25 & 79.05 & 37.80 & 60.99 & 86.93 \\
 & QuaRot & 47.70 & 74.41 & 70.82 & 65.35 & 75.14 & 83.09 & 39.00 & 65.07 & 92.65 \\
 & FlatQuant & 50.17 & 72.94 & 71.71 & 65.82 & 74.54 & 84.19 & 40.40 & 65.68 & 93.83 \\
  & SpinQuant & 47.95 & 75.34 & 71.89 & 66.77 & 75.79 & 83.58 & 38.20 & 65.65 & 93.28 \\
 & MR-GPTQ & 51.79 & 76.56 & 72.28 & 65.67 & 75.19 & 83.21 & 39.20 & 66.27 & 94.50 \\
 \cdashline{2-11}
\addlinespace[0.3em]
 & \textbf{\MN{}-LU (Ours)} & 52.73 & 75.55 & 72.76 & 69.22 & 76.22 & 83.76 & 40.00 & \textbf{67.18} & \textbf{95.92} \\
 & \textbf{\MN{}-QR (Ours)} & 53.16 & 75.80 & 72.45 & 68.51 & 75.79 & 82.91 & 38.40 & 66.71 & 95.10 \\ 
 \bottomrule
\end{tabular}%
}
\end{table*}

==> files/tables/results_bench.tex <==
\begin{table*}[t]
\caption{Benchmark accuracy (\%) with dashed separators after Float baselines. Best results per model are highlighted in bold.}
\centering
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{llccccccc}
\toprule
Model & Method & WinoGrande & HellaSwag & PIQA & OBQA & ARC-E & ARC-C & Avg. \\
\midrule

\multirow{5}{*}{Llama3.2-1B-Instruct}
& Float            & 61.24 & 61.51 & 74.64 & 37.60 & 63.84 & 59.22 & 59.68 \\
\cdashline{2-9}
& MR-GPTQ Results  & 58.72 & 54.89 & 70.40 & 33.40 & 46.34 & 0.00  & 43.96 \\
& MR-GPTQ Recovery & 95.38 & 91.33 & 94.32 & 88.83 & 72.59 & 0.00  & 73.74 \\
& Ours Results     & 59.51 & 57.09 & 72.19 & 35.60 & 59.63 & 21.63 & 50.94 \\
& Ours Recovery    & \textbf{97.18} & \textbf{92.81} & \textbf{96.72} & \textbf{94.68} & \textbf{93.41} & \textbf{36.52} & \textbf{85.22} \\

\midrule
\multirow{5}{*}{Llama3.2-3B-Instruct}
& Float            & 67.63 & 71.44 & 75.95 & 40.80 & 71.30 & 78.63 & 67.63 \\
\cdashline{2-9}
& MR-GPTQ Results  & 68.03 & 70.08 & 74.05 & 40.00 & 66.16 & --    & 63.66 \\
& MR-GPTQ Recovery & 97.06 & 95.43 & 97.50 & 98.04 & 92.79 & --    & 96.16 \\
& Ours Results     & 65.66 & 69.57 & 74.21 & 38.60 & 67.97 & --    & 63.20 \\
& Ours Recovery    & \textbf{97.09} & \textbf{97.38} & \textbf{97.71} & \textbf{94.61} & \textbf{95.33} & --    & \textbf{96.42} \\

\midrule
\multirow{5}{*}{Llama3.1-8B-Instruct}
& Float            & 76.08 & 78.51 & -- & -- & -- & -- & -- \\
\cdashline{2-9}
& MR-GPTQ Results  & 74.90 & 77.00 & -- & -- & -- & -- & 75.95 \\
& MR-GPTQ Recovery & \textbf{96.10} & 96.25 & -- & -- & -- & -- & 96.18 \\
& Ours Results     & 72.61 & 76.17 & -- & -- & -- & -- & 74.39 \\
& Ours Recovery    & {95.44} & \textbf{97.02} & -- & -- & -- & -- & \textbf{96.23} \\

\midrule
\multirow{7}{*}{Llama3.2-1B}
& Float            & 62.98 & 65.78 & 74.81 & 37.40 & 61.91 & -- & -- \\
\cdashline{2-9}
& BRQ Results      & 55.88 & NA & 70.46 & 34.20 & 55.47 & 33.36 & 49.87 \\
& BRQ Recovery     & 92.19 & NA & 94.82 & 91.93 & 91.73 & 92.00 & 92.53 \\
& MR-GPTQ Results  & 59.35 & 59.75 & 70.08 & 35.00 & 58.38 & -- & 56.51 \\
& MR-GPTQ Recovery & 94.24 & 90.83 & 93.68 & 93.58 & 94.30 & -- & 93.33 \\
& Ours Results     & 57.62 & 60.18 & 70.78 & 34.80 & 57.07 & -- & 56.09 \\
& Ours Recovery    & \textbf{91.49} & \textbf{91.49} & \textbf{94.61} & \textbf{93.05} & \textbf{92.18} & -- & \textbf{92.56} \\

\midrule
\multirow{7}{*}{Llama3.2-3B}
& Float            & 72.14 & 76.77 & 76.39 & 40.80 & 71.80 & -- & -- \\
\cdashline{2-9}
& BRQ Results      & 62.59 & NA & 75.35 & 38.60 & 67.42 & 40.44 & 56.88 \\
& BRQ Recovery     & 90.22 & NA & 94.95 & 88.94 & 94.12 & 87.77 & 91.20 \\
& MR-GPTQ Results  & 67.25 & 73.08 & 75.57 & 40.20 & 66.50 & -- & 64.52 \\
& MR-GPTQ Recovery & 93.22 & 95.19 & 98.93 & 98.53 & 92.62 & -- & 95.70 \\
& Ours Results     & -- & 72.93 & 75.24 & 39.00 & 69.07 & -- & 64.06 \\
& Ours Recovery    & -- & \textbf{95.00} & \textbf{98.49} & \textbf{95.59} & \textbf{96.20} & -- & \textbf{96.32} \\

\midrule
\multirow{5}{*}{Qwen3-8B}
& Float            & 70.17 & 76.53 & 76.66 & 41.60 & 80.68 & 56.74 & -- \\
\cdashline{2-9}
& MR-GPTQ Results  & 68.03 & 73.55 & 74.97 & 41.40 & 79.55 & 54.44 & 65.32 \\
& MR-GPTQ Recovery & 97.39 & 96.41 & 97.80 & 99.52 & 98.60 & 95.95 & 97.61 \\
& Ours Results     & 68.35 & 73.75 & 75.41 & -- & 77.78 & 54.35 & 69.93 \\
& Ours Recovery    & \textbf{97.41} & \textbf{96.37} & \textbf{98.37} & -- & \textbf{96.41} & \textbf{95.79} & \textbf{96.87} \\

\bottomrule
\end{tabular}
\label{tab:quant_results}
\end{table*}

==> includes/base.tex <==
\usepackage{ifthen}
\newboolean{edit}
\setboolean{edit}{true}
\newcommand{\editenable}[1]{\setboolean{edit}{true}}
\newcommand{\editdisable}[1]{\setboolean{edit}{false}}

\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{algorithm}
\usepackage{amsmath}
\usepackage{cite}
\usepackage{acronym}

\usepackage{commath,amsmath,amssymb,amsfonts}

% \usepackage{changes}
\usepackage{accents}
\usepackage[inkscapearea=page]{svg}

\usepackage{mathtools}
\usepackage{hyperref}
\usepackage{amssymb}
\usepackage{bm}
\usepackage{graphicx}
\usepackage{float}
\usepackage{amsmath}
\usepackage{tikz}
\usepackage{multicol}
\usepackage{dsfont}
\usepackage{tcolorbox}
% \usepackage{subcaption}
\usepackage{bbm}
\usepackage{multirow}
\usetikzlibrary{positioning, backgrounds, fit, shapes.arrows}
\usetikzlibrary{decorations.markings}
% \usepackage{amsthm}
% \usepackage{enumitem}
\usepackage{cuted}
\setlength\stripsep{3pt plus 1pt minus 1pt}
\let\labelindent\relax
\usepackage{enumitem}
\usepackage{caption}
\usepackage{booktabs}
% \usepackage{clipboard}
\usepackage{subcaption}
\captionsetup{compatibility=false}

% \theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem*{problem}{Problem Statement}
\newtheorem{assumption}{Assumption}[section]
\newtheorem{remark}{Remark}
% \usepackage{caption}

\usepackage{algorithm}
\usepackage{algpseudocode}
\tikzset{block/.style = {draw, fill=white, rectangle,
		minimum height=3em, minimum width=2cm},
	input/.style = {coordinate},
	output/.style = {coordinate},
	pinstyle/.style = {pin edge={to-,t,black}}
	radiation/.style={{decorate,decoration={expanding waves,angle=90,segment   length=4pt}}}
	
}
\usepackage{smartdiagram}

\tikzstyle{block} = [draw, rectangle, minimum height=2em, minimum width=2em]
\tikzstyle{sum} = [draw, circle,minimum width=0.1 cm]
\tikzstyle{input} = [coordinate]
\tikzstyle{output} = [coordinate]
\tikzstyle{dummy} = [coordinate]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\usetikzlibrary{positioning, fit, arrows.meta}
\usetikzlibrary{positioning}
\usetikzlibrary{shapes,arrows}
\tikzstyle{frame_cyan} = [thick, draw=blue, solid,inner sep=0.3em]
\tikzstyle{frame_red} = [thick, draw=red, solid,inner sep=0.3em]
\tikzstyle{frame_green} = [thick, draw=green, solid,inner sep=0.3em]
\DeclareMathOperator{\ReLU}{ReLU}
\newcommand{\KL}{\ensuremath{\mathrm{KL}}}
\newcommand{\Ber}{\ensuremath{\mathrm{Ber}}}
 
\usepackage{tikz}
\usepackage{xcolor}
\definecolor{fc}{HTML}{1E90FF}
\definecolor{h}{HTML}{228B22}
\definecolor{bias}{HTML}{87CEFA}
\definecolor{noise}{HTML}{8B008B}
\definecolor{conv}{HTML}{FFA500}
\definecolor{pool}{HTML}{B22222}
\definecolor{up}{HTML}{B22222}
\definecolor{view}{HTML}{FFFFFF}
\definecolor{bn}{HTML}{FFD700}
\tikzset{fc/.style={black,draw=black,fill=fc,rectangle,minimum height=1cm}}
\tikzset{h/.style={black,draw=black,fill=h,rectangle,minimum height=1cm}}
\tikzset{bias/.style={black,draw=black,fill=bias,rectangle,minimum height=1cm}}
\tikzset{noise/.style={black,draw=black,fill=noise,rectangle,minimum height=1cm}}
\tikzset{conv/.style={black,draw=black,fill=conv,rectangle,minimum height=1cm}}
\tikzset{pool/.style={black,draw=black,fill=pool,rectangle,minimum height=1cm}}
\tikzset{up/.style={black,draw=black,fill=up,rectangle,minimum height=1cm}}
\tikzset{view/.style={black,draw=black,fill=view,rectangle,minimum height=1cm}}
\tikzset{bn/.style={black,draw=black,fill=bn,rectangle,minimum height=1cm}}
 
\usepackage{xspace}
\newcommand*{\eg}{\emph{e.g.}\@\xspace}
\newcommand*{\Eg}{\emph{E.g.}\@\xspace}
\newcommand*{\ie}{\emph{i.e.}\@\xspace}
\newcommand*{\etc}{\emph{etc.}\@\xspace}
\newcommand*{\etal}{\emph{et al.}\@\xspace}
\newcommand*{\cf}{\emph{cf.}\@\xspace}
\newcommand*{\vs}{\emph{vs.}\@\xspace}

%%%%%%%%%%%%%%%%%%
% Tikz Commands
%%%%%%%%%%%%%%%%%%
\tikzstyle{dummy} = [coordinate]
\pgfkeys{/pgf/.cd,
  parallelepiped offset x/.initial=2mm,
  parallelepiped offset y/.initial=2mm
}
\pgfdeclareshape{parallelepiped}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \backgroundpath{
    % store lower right in xa/ya and upper right in xb/yb
    \southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
    \northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
    \pgfmathsetlength\pgfutil@tempdima{\pgfkeysvalueof{/pgf/parallelepiped offset x}}
    \pgfmathsetlength\pgfutil@tempdimb{\pgfkeysvalueof{/pgf/parallelepiped offset y}}
    \def\ppd@offset{\pgfpoint{\pgfutil@tempdima}{\pgfutil@tempdimb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xa}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathlineto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathclose
    \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@ya}}
    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@ya}}{\ppd@offset}}
    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\ppd@offset}}
    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xa}{\pgf@yb}}{\ppd@offset}}
    \pgfpathlineto{\pgfqpoint{\pgf@xa}{\pgf@yb}}
    \pgfpathmoveto{\pgfqpoint{\pgf@xb}{\pgf@yb}}
    \pgfpathlineto{\pgfpointadd{\pgfpoint{\pgf@xb}{\pgf@yb}}{\ppd@offset}}
  }
}
% https://tex.stackexchange.com/a/103691/121799
\pgfdeclareshape{document}{
\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{north east}
\inheritanchor[from=rectangle]{north west}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{south east}
\inheritanchor[from=rectangle]{south west}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{east}
\backgroundpath{%
\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
\pgf@xc=\pgf@xb \advance\pgf@xc by-5pt % this should be a parameter
\pgf@yc=\pgf@ya \advance\pgf@yc by5pt
\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@ya}}
\pgfpathclose
% add little corner
\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yc}}
\pgfpathclose
}
}
\tikzstyle{block} = [draw, fill=white, rectangle, 
    minimum height=3em, minimum width=6em]
    
\usetikzlibrary{backgrounds}
\usepackage{pifont}% http://ctan.org/pkg/pifont
%\usepackage[table,xcdraw]{xcolor}
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=2cm, minimum height=0.7cm,text centered, draw=black, fill=lime!30]
% \usepackage{biblatex}
\usepackage{stackengine}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Alg Phase
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\makeatletter
\newcounter{phase}[algorithm]
\newlength{\phaserulewidth}
\newcommand{\setphaserulewidth}{\setlength{\phaserulewidth}}
\newcommand{\phase}[1]{%
  \vspace{-1.25ex}
  % Top phase rule
  \Statex\leavevmode\llap{\rule{\dimexpr\labelwidth+\labelsep}{\phaserulewidth}}\rule{\linewidth}{\phaserulewidth}
  \Statex\strut\refstepcounter{phase}\textit{Phase~\thephase~--~#1}% Phase text
  % Bottom phase rule
  \vspace{-1.25ex}\Statex\leavevmode\llap{\rule{\dimexpr\labelwidth+\labelsep}{\phaserulewidth}}\rule{\linewidth}{\phaserulewidth}}
\makeatother
\setphaserulewidth{.7pt}
\makeatother
\usepackage{colortbl}

==> includes/base_editing.tex <==

\ifthenelse{\boolean{edit}}{%
  % This code will be executed if x is true
  \usepackage{todonotes}
  \usepackage{color-edits} % [suppress]
}{%
  % This code will be executed if x is false
  \usepackage[disable]{todonotes}
  \usepackage[suppress]{color-edits} % [suppress]
}
